Understanding Deep Generative Models with Generalized Empirical Likelihoods

Understanding how well a deep generative model captures a distribution of high-dimensional data remains an important open challenge. It is especially difficult for certain model classes, such as Generative Adversarial Networks and Diffusion Models, whose models do not admit exact likelihoods. In this work, we demonstrate that generalized empirical likelihood (GEL) methods offer a family of diagnostic tools that can identify many deficiencies of deep generative models (DGMs). We show, with appropriate specification of moment conditions, that the proposed method can identify which modes have been dropped, the degree to which DGMs are mode imbalanced, and whether DGMs sufficiently capture intra-class diversity. We show how to combine techniques from Maximum Mean Discrepancy and Generalized Empirical Likelihood to create not only distribution tests that retain per-sample interpretability, but also metrics that include label information. We find that such tests predict the degree of mode dropping and mode imbalance up to 60% better than metrics such as improved precision/recall. We provide an implementation at https://github.com/deepmind/understanding_deep_generative_models_with_generalized_empirical_likelihood/.

==> figures/single_slide_convex_hull_one_pane.tex <==
\begin{figure*}[t]
\centering
\setlength{\tabcolsep}{3pt}
\begin{tabular}{ccc|ccc}
\toprule
\multicolumn{3}{c}{One-sample} & \multicolumn{3}{c}{Two-sample} \\
\midrule
Empirical & Reverse & Euclidean & Empirical & Reverse & Euclidean\\
Likelihood & KL & Likelihood & Likelihood & KL & Likelihood\\
\midrule
\begin{minipage}{0.13\textwidth}
\includegraphics[width=\linewidth, trim=0 0 480 0, clip]{figures/convex_hull/single_slide_convex_hull.png}
\end{minipage}
&
\begin{minipage}{0.13\textwidth}
\includegraphics[width=\linewidth, trim=240 0 240 0, clip]{figures/convex_hull/single_slide_convex_hull.png}
\end{minipage}
&
\begin{minipage}{0.13\textwidth}
\includegraphics[width=\linewidth, trim=480 0 0 0, clip]{figures/convex_hull/single_slide_convex_hull.png}
\end{minipage}
&
\begin{minipage}{0.14\textwidth}
\includegraphics[width=\linewidth]{figures/convex_hull/convex_hull_two_sample_el.png}
\end{minipage} &

\begin{minipage}{0.14\textwidth}
\includegraphics[width=\linewidth]{figures/convex_hull/convex_hull_two_sample_et.png}
\end{minipage} &
\begin{minipage}{0.14\textwidth}
\includegraphics[width=\linewidth]{figures/convex_hull/convex_hull_two_sample_euc.png}
\end{minipage}
\\
\bottomrule
\end{tabular}
\caption{Illustration of the convex hull condition for one- and two-sample generalized empirical likelihood. For one-sample empirical likelihood to be finite, the $\mu$ vector must lie in the interior of the convex hull (top left). For the reverse KL to be finite, $\mu$ must lie in the interior or on the boundary of the convex hull (top middle). For two-sample empirical likelihood to be finite, the intersection of the interior of the two convex hulls must be non-empty (bottom left). For two-sample reverse KL to be finite, the intersection of the closure of the two convex hulls must be non-empty (bottom middle). Euclidean Likelihoods are always finite (top and bottom right).}
\label{fig:convex_hull}
\setlength{\tabcolsep}{6pt}
\end{figure*}
